Latent Space Dynamics Identification for Interface Tracking with Application to Shock-Induced Pore Collapse

Capturing sharp, evolving interfaces remains a central challenge in reduced-order modeling, especially when data is limited and the system exhibits localized nonlinearities or discontinuities. We propose LaSDI-IT (Latent Space Dynamics Identification for Interface Tracking), a data-driven framework that combines low-dimensional latent dynamics learning with explicit interface-aware encoding to enable accurate and efficient modeling of physical systems involving moving material boundaries. At the core of LaSDI-IT is a revised auto-encoder architecture that jointly reconstructs the physical field and an indicator function representing material regions or phases, allowing the model to track complex interface evolution without requiring detailed physical models or mesh adaptation. The latent dynamics are learned through linear regression in the encoded space and generalized across parameter regimes using Gaussian process interpolation with greedy sampling. We demonstrate LaSDI-IT on the problem of shock-induced pore collapse in high explosives, a process characterized by sharp temperature gradients and dynamically deforming pore geometries. The method achieves relative prediction errors below 9% across the parameter space, accurately recovers key quantities of interest such as pore area and hot spot formation, and matches the performance of dense training with only half the data. This latent dynamics prediction was 106 times faster than the conventional high-fidelity simulation, proving its utility for multi-query applications. These results highlight LaSDI-IT as a general, data-efficient framework for modeling discontinuity-rich systems in computational physics, with potential applications in multiphase flows, fracture mechanics, and phase change problems.

==> packages.tex <==
\usepackage{amssymb, amsmath}
\usepackage{stmaryrd}

\usepackage{hyperref}

\usepackage{comment}
% \usepackage{arydshln}
\usepackage{bm}
\usepackage[textsize=tiny,
disable
]{todonotes}

\usepackage{tikz}
\usetikzlibrary{positioning}
% \usepackage{pgfplotstable}
\usepackage{pgfplots}
% \usepgfplotslibrary{external} 
% \tikzexternalize
\pgfplotsset{compat=1.10}
\usepgfplotslibrary{groupplots,fillbetween}
\usetikzlibrary{spy, backgrounds}
\usetikzlibrary{shapes.geometric, arrows.meta}

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFaddtex}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdeltex}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF HYPERREF PREAMBLE %DIF PREAMBLE
\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

==> sections_abstract.tex <==
% \begin{abstract}
High explosives (HEs) and their detonation properties have been an important field of study
for various applications such as solid rocket propellants, insensitive munitions, tunnel constructions and demolition.
Shock-induced collapse of pores in microstructures is a key mechanism of developing hot spots and initiating chemical reaction of detonation.
However, numerical modeling of complex pore collapse process is limited to micro scales due to computational cost of high-fidelity models.
There is a strong need for a surrogate pore collapse model that may provide efficient predictions,
thereby accelerating design process of high explosives.
In this work,
we study the use of Gaussian-process-based latent dynamics identification (GPLaSDI)
for pore collapse process.
The GPLaSDI framework combines autoencoders for low-dimensional latent space extraction,
sparse identification of latent dynamics,
and Gaussian process-based parametric interpolation with greedy sampling.
The framework is applied to simulate the collapse of single oval-shaped pores,
parameterized by their major axis length and angle.
A revised autoencoder architecture is introduced to track both temperature fields and pore boundaries,
addressing challenges posed by discontinuities at the pore interface.
This enables accurate predictions of key metrics such as hot spot area, pore area, and maximum temperature.
Using greedy sampling, the GPLaSDI framework achieves comparable accuracy to uniformly sampled training data,
but with significantly reduced data requirements.
The trained latent dynamics model accurately captures the evolution of pore collapse and hot spot formation,
providing detailed predictions of instantaneous temperature fields with a relative error of $\lesssim9\%$
in all test cases.
This study demonstrates the potential of data-driven latent dynamics modeling
to accelerate HE material design and analysis,
while reducing reliance on computationally expensive simulations.
% \end{abstract}


==> sections_ae.tex <==
\section{Autoencoder design}\label{sec:ae}

The design of the autoencoder is a critical component of the GPLaSDI framework,
as it determines how effectively the high-dimensional temperature field data is
compressed into a low-dimensional latent space while preserving key features.
This section explores the challenges of applying standard autoencoder architectures
to the pore collapse problem and introduces a revised autoencoder design that addresses these challenges.

\subsection{Limitations with the standard autoencoder}\label{subsec:vanilla}
Initially, the standard autoencoder architecture was investigated to reconstruct the temperature field.
A multilayer perceptron (MLP) with depth $L$ is used,
\begin{equation}
NN(\bq;\theta) = \left( \cT_{L+1}\circ \sigma \circ \cT_L \circ \cdots \circ \sigma \circ \cT_1 \right)(\bq;\theta),
\end{equation}
for a general vector $\bq\in\rR^{d}$,
where each layer $\cT_k: \rR^{d_{k-1}}\to\rR^{d_k}$ is an affine function
\begin{equation}
\bq_k \equiv \cT_k(\bq_{k-1}) = \bW_k\bq_{k-1} + \bb_k,
\end{equation}
and $\sigma$ is softplus activation function.
The NN parameter is composed of weight matrices and bias vectors of all layers,
i.e. $\theta = \{\bW_1, \bb_1, \ldots, \bW_{L+1}, \bb_{L+1}\}$.
For encoder (\ref{eq:en}),
a $L=6$ MLP with layer widths $(d_0, d_1, \ldots, d_7) = (N_x, 3000, 300, 300, 100, 100, 30, N_z)$ is employed.
For decoder (\ref{eq:de}),
a $L=6$ MLP with the same layer widths in reverse order is used.
\par
To evaluate the reconstruction ability of the autoencoder,
it is trained with the objective (\ref{eq:J}) with $\beta_1=0$.
The training is performed using the ADAM optimizer~\cite{kingma2014adam} for $10^4$ iterations
with a learning rate of $10^{-4}$.
The training dataset consists of $N_p=4$ parameter points:
$\{(\deg{0}, 1\mu m), (\deg{20}, 1\mu m), (\deg{0}, 1.2\mu m), (\deg{20}, 1.2\mu m)\}$.
\par
\begin{figure}[tbph]
    \input{figures_vanilla_ae.tex}
    \caption{(a) Reconstruction of the temperature field with the standard AE, and (b) its point-wise error.}
    \label{fig:vanilla-ae}
\end{figure}
This standard architecture, however,
struggles to accurately embed the pore shape into the latent space.
Figure~\ref{fig:vanilla-ae} shows a reconstruction of HE temperature field
using the trained autoencoder with a latent dimension $N_z=10$.
The AE reconstruction in Figure~\ref{fig:vanilla-ae}~(a)
captures the complex features of temperature field fairly well in most of the domain.
However, as shown in Figure~\ref{fig:vanilla-ae}~(b),
significantly high error is localized near the pore interface,
indicating that the AE failed to accurately capture the pore boundary.
Furthermore, the reconstructed pore region exhibits non-zero temperature values.
Since some of these values are unphysical, we may be able to assume this region as the pore region.
However, there are also temperatures near a room temperature,
which are ambiguous for determining the pore boundary.
This failure compromised the accurate determination of the pore area---an
essential metric in HE material design.
Various neural network sizes, depths, and alternative architectures, such as convolutional neural networks,
were tested, but the results remained similar.
\par
The primary challenge stems from the sharp discontinuity in temperature field
across the pore boundary, as shown from Figure~\ref{fig:he-temp}.
From a spectral viewpoint,
resolving such discontinuities requires capturing all spatial wavenumber modes.
However, NN is well known for its spectral bias~\cite{rahaman2019spectral},
where high frequency features are trained much slower than low frequency counterparts.
The autoencoder likewise suffer from spectral bias,
having difficulty in resolving the sharp discontinuity at the pore boundary.
A deeper and wider NN may be able to resolve the discontinuity,
though it also increases the training iteration and time.
\par
For accurate pore detection, the architecture of the autoencoder must be revised.
There are many novel NN architectures and training methods proposed to tackle the spectral bias of NN,
such as multi-stage NN~\cite{wang2024multi} and Fourier feature let NN~\cite{tancik2020fourier}.
Our goal in this study, however, is not to tackle the spectral bias of NN and to perfectly resolve the sharp discontinuity.
The root cause of the failure is that the autoencoder is trained to capture $0K$ value
as part of the temperature field,
though it is rather an indication that the grid point belongs to the pore.
In this study, we revise the autoencoder to track both the temperature field
and the HE domain region, which is described subsequently.

\subsection{Revised Autoencoder architecture}
We introduce an indicator variable for HE domain,
\begin{equation}
\bphi(T(\bx; \bp)) = \mathbf{1}_{T>0}(\bx; \bp),
\end{equation}
where $\bphi$ equals 1 in the HE domain and 0 in the pore region.
\par
The revised autoencoder was designed to simultaneously capture the temperature field
and the HE domain using this indicator variable.
Specifically,
the decoder now decodes both the (scaled) temperature field and the indicator variable
from the latent space variable,
\begin{equation}\label{eq:de1}
(\tilde{T}', \bphi_{pred}) = \De(\bz; \theta_{de}).
\end{equation}
The same MLP architecture in Section~\ref{subsec:vanilla} can be used,
though the last output layer width is doubled to accommodate both outputs:
$(d_0, d_1, \ldots, d_7) = (N_z, 30, 100, 100, 300, 300, 3000, 2N_x)$.
To ensure the decoded indicator $\bphi_{pred}$ to range from 0 to 1,
a sigmoid activation function $\sigma_{sig}$ was applied to the last layer,
\begin{equation}
\begin{pmatrix}
\tilde{T}'\\ \bphi_{pred}
\end{pmatrix}
\equiv \cT_{L+1}(\bq_L)
=
\begin{pmatrix}
\bW_{L+1}\bq_L + \bb_{L+1}\\ \sigma_{sig}(\bW'_{L+1}\bq_L + \bb'_{L+1})
\end{pmatrix}.
\end{equation}
The decoded temperature field $\tilde{T}'$ is defined over the entire domain,
not necessarily tracking the pore region.
The decoded indicator $\bphi_{pred}\in[0, 1]^{N_x}$ essentially serves as
a probability for a grid point to be in HE domain.
The final reconstructed temperature field $\tilde{T}_{pred}$
is computed combining $\tilde{T}'$ and $\bphi_{pred}$,
\begin{equation}\label{eq:Tpred1}
\tilde{T}_{pred}(\bx; \bp) = \tilde{T}'(\bx; \bp) \times \mathbf{1}_{\bphi_{pred}>0.5}(\bx; \bp).
\end{equation}
This formulation ensured that the reconstructed temperature field was zero in regions where $\bphi_{pred}<=0.5$,
regardless of the value of $\tilde{T}'$.
As long as $\bphi_{pred}$ was reconstructed accurately,
the temperature field within the pore region did not need to match (the scaled value of) $0K$ exactly.
\par
\begin{figure*}[htbp]
    \input{figures_ae_architecture.tex}
    \caption{Schematic of autoencoder architecture.\YC{The output size of decoder needs to be twice as big as the input size of the encoder.}}
    \label{fig:ae-architecture}
\end{figure*}
While the encoder could also be modified to take $\bphi$ as an input,
experiments showed that the encoder performed better when taking the temperature field $T$ solely as an input.
\todo{Add these results as appendix?}
% In fact, several encoder architectures that take $\bphi$ as an input are tested,
% though none of them could be trained better than the architecture in Figure~\ref{fig:ae-architecture}.
The rationale is that the autoencoder must be capable of extracting $\bphi$ out of $T$,
since $\bphi$ is essentially a filtered information of $T$.
The architecture of the revised autoencoder is illustrated in Figure~\ref{fig:ae-architecture}.

\subsection{Revised autoencoder loss}
We denote as $\bphi_k(\bp_i)$ the indicator corresponding
to the training data temperature field $T_k(\bp_i)$ at time step $k$ for the parameter $\bp_i$.
The reconstruction of training data $\tilde{T}_{k,pred}(\bp_p)$
and $\bphi_{k, pred}(\bp_p)$ are evaluated as
\begin{equation}
\begin{pmatrix}
\tilde{T}_{k,pred}(\bp_p) \\
\bphi_{k, pred}(\bp_p)
\end{pmatrix}
=
\De(\En(T_k(\bp_p); \theta_{en}); \theta_{de}).
\end{equation}
The autoencoder loss (\ref{eq:J-ae0}) is now revised to track
both $\tilde{T}_{pred}$ and $\bphi_{pred}$,
\begin{subequations}\label{eq:J-ae1}
\begin{equation}
\cJ_{AE} = \cJ_{val} + \cJ_{mask},
\end{equation}
which is composed of value loss $\cJ_{val}$ and mask loss $\cJ_{mask}$,
\begin{equation}\label{eq:J-value}
\cJ_{val} = \frac{1}{N_pN_tN_x}\sum_p^{N_p}\sum_k^{N_t}
\Vert \tT_k(\bp_p) - \tilde{T}_{k,pred}(\bp_p) \Vert^2
\end{equation}
\begin{equation}\label{eq:J-mask}
\cJ_{mask} = \frac{1}{N_pN_tN_x}\sum_p^{N_p}\sum_k^{N_t}
\Vert \bphi_k(\bp_p) - \bphi_{k, pred}(\bp_p) \Vert^2.
\end{equation}
\end{subequations}

\subsection{Revised scaling of the temperature field}
Since the temperatures in the pore region is not an actual temperature but an indicator,
the temporal average and standard deviation in (\ref{eq:T-scale0}) need not count
these $0K$ values in the pore region.
Thus we count the sample size of HE temperature at each grid point of the training data,
\begin{equation}
N_{HE}(\bx_g) = \frac{1}{N_pN_t}\sum_{p=1}^{N_p}\sum_{k=1}^{N_t}\bphi_k(\bx_g; \bp_p) \in \rR^{N_x},
\end{equation}
and evaluate average and standard deviation only for non-zero HE temperature values,
\begin{subequations}\label{eq:T-scale1}
\begin{equation}
\overline{T}(\bx_g) = \frac{1}{N_{HE}(\bx_g)}\frac{1}{N_pN_t}\sum_{p=1}^{N_p}\sum_{k=1}^{N_t}T_k(\bx_g; \bp)\bphi_k(\bx_g; \bp_p)
\end{equation}
\begin{equation}
\begin{split}
\std[T](\bx_g) = &\left\{ \frac{1}{N_{HE}(\bx_g)}\frac{1}{N_pN_t}\sum_{p=1}^{N_p}\sum_{k=1}^{N_t} \right.\\
&\qquad (T_k(\bx_g; \bp)\bphi_k(\bx_g; \bp_p) - \overline{T}(\bx_g))^2 \bigg\}^{1/2}.
\end{split}
\end{equation}
\end{subequations}
\par
\begin{figure}[tbph]
    \input{figures_ae_scaling.tex}
    \caption{Temporal (a) average and (b) standard deviation of HE temperature ($K$) for 36-case training data.}
    \label{fig:ae-scaling}
\end{figure}
Figure~\ref{fig:ae-scaling} shows the average and standard deviation in (\ref{eq:T-scale1})
for a training dataset of $N_p=36$ parameter points.
The parameter points are uniformly spaced as a $6\times6$ array in the range of $[\deg{0}, \deg{20}]\times[1\mu m, 1.2\mu m]$.
The initial pore shape distinctly appears in both the average and the standard deviation.
High variance is observed downstream of the initial pore location,
where the hot spot is being developed and ejected out of the pore collapse process.
We note that the average within the pore region exhibits high temperature
due to hot spot development following the pore collapse,
while the variance within the initial pore region is significantly low.
\refC{These} statistics cannot be captured well with the standard scaling in (\ref{eq:T-scale0}):
as all the $0K$ values are included, the temperature variance appears to be high in the pore region,
though it is not in reality.

\subsection{Reconstruction results with the revised autoencoder}
To compare with the standard autoencoder,
the revised model is trained for the same $N_p=4$-parameter-points training data in Section~\ref{subsec:vanilla}.
The revised scaling (\ref{eq:T-scale1}) is applied,
and the revised autoencoder loss (\ref{eq:J-ae1}) is minimized with ADAM optimizer at the same learning rate $10^{-4}$
for $10^4$ iterations.
The same hidden layers are used for both the encoder and the decoder.
\par
\begin{figure}[tbph]
    \input{figures_ae_loss.tex}
    \caption{Loss history of the standard AE and revised AE.}
    \label{fig:ae-loss}
\end{figure}
Figure~\ref{fig:ae-loss} shows the loss history of the revised AE,
compared to the standard one in Section~\ref{subsec:vanilla}.
The mask loss (\ref{eq:J-mask}) of the revised AE
is minimized by approximately four orders of magnitude.
The value loss (\ref{eq:J-value}) of the revised AE
also achieved a similar reduction,
which is much faster than the loss (\ref{eq:J-ae0}) of the standard AE.
\begin{figure}[tbph]
    \input{figures_revised_ae.tex}
    \caption{(a) Reconstruction of the temperature field with the revised AE, and (b) its point-wise error.}
    \label{fig:revised-ae}
\end{figure}
Figure~\ref{fig:revised-ae} shows the reconstruction of the temperature field by the revised AE.
Compared to the standard AE, almost no high-temperature error near the pore boundary is observed.
Furthermore, the pore region is properly marked out with $0K$ without any ambiguity in pore region determination.
\par
Although the revised loss (\ref{eq:J-ae1}) is essentially a multi-objective minimization,
its result was significantly better than the standard single-objective minimization.
There are mainly two factors contributing to this improved training.
First, minimizing the mask loss (\ref{eq:J-mask}) can be considered
as a classification at each grid point,
which is easier than matching $0K$ values in the pore region as a regression problem.
Second, $0K$ values in the pore region are removed from the statistics,
significantly decreasing the temperature variance within the pore region.
By tracking both temperature and indicator,
the decoded temperature $\tilde{T}'$ in (\ref{eq:Tpred1})
needs to resolve only the HE temperature statistics with small variance,
not $0K$ values which outlies far beyond the statistics.
\par
For the overall LaSDI framework, the revised autoencoder with the architecture specified in this section is
adopted throughout this study.


==> sections_intro.tex <==
% \section{\label{sec:level1}First-level heading:\protect\\ The line
% break was forced \lowercase{via} \textbackslash\textbackslash}
\section{Introduction}\label{sec:intro}

Understanding the physical mechanisms governing
the shock initiation of high explosives (HEs)
is an important yet challenging endeavor.
These materials are widely used in both civil and military applications
to release large quantities of energy over short periods of time.
HEs are often composed of energetic crystals held together with a polymer binder,
which are inherently heterogeneous.
Many factors, including variations in particle sizes, material concentrations,
and microscopic defects can all affect the ignition behavior of an HE.
To minimize the risk of unintended ignition or detonation
in potential accident scenarios,
a better understanding of early ignition behavior is required.
\par
One of the primary theories describing the ignition behavior of HEs
under shock loading focuses on the idea of ``hot spots''~\cite{bowden1985initiation}.
Hot spot area of the HE can rapidly heat up to critically high temperatures
due to localized energy dissipation under shock loading.
Major factors of temperature rise involve
plastic deformation and material jetting, frictional heating,
viscous heating, and shear banding~\cite{fried2012role,tarver1996critical,field1992hot}.
As the temperature increases, the rate of chemical kinetics increases,
causing the HE material to more rapidly decompose into its product species.
This generation of gases under high pressures exerts itself
onto the surrounding material, potentially generating new hot spots and
initiating a self-sustaining detonation wave behind the initial shock compression wavefront.
This detonation wave propagates more rapidly through the compressed material,
eventually overtaking the initial shock wave and leading to uncontrolled thermal runaway. 
\par
Voids in HE materials are common locations for hot spot formation~\cite{menikoff2004pore,nesterenko1994instability}.
These pockets of empty space are defects in the crystal
which provide little resistance to the oncoming shock wave.
The resulting plastic deformation and jetting of the HE undergoing pore collapse
has been widely studied over the years
to attempt to predict hot spot formation~\cite{austin2014modeling,miller2019ignition,miller2021probabilistic,kapahi2015three}.
\par
With recent advance in high performance computing,
numerical methods now provide high-fidelity predictions for
complex hydrodynamics of pore collapse dynamics~\cite{noble2017ale3d}.
However, realistic pores come in a variety of shapes and sizes,
and simulating the collapse of each of them would be computationally infeasible.
Furthermore, the modeling and design process of HEs
would require solving of an inverse problem or design optimization,
which involve multiple queries of simulation.
\todo{Chris/Keo, can you confirm/correct this motivation for reduced order model?}
High-fidelity HPC simulations of realistic pore collapses
are computationally expensive, even for one configuration,
making them impractical for multi-query applications.
A fast-running framework for predicting hot spot temperature due to pore collapse
is therefore required to effectively analyze real materials and make usable predictions
as to the likelihood of HE ignition.
\par
Reduced order modeling (ROM) has been the focus of numerous research efforts
across engineering and science applications.
ROM aims to develop a surrogate model
that would effectively approximate essential features of complex physics,
thereby enabling computationally cheaper prediction with modest accuracy.
One of the widely used ROM approach is projection-based ROM,
where high-fidelity numerical models of the underlying physics
is projected onto a low-dimensional subspace.
The low-dimensional subspace can be identified from data
in various methods, from linear subspace
techniques~\cite{berkooz1993proper,safonov2002schur,rozza2008reduced}
to nonlinear compression approaches such as autoencoders~\cite{lee2020model,kim2022fast}.
All these approaches are considered intrusive
because they involve in-depth manipulation of the underlying governing equations
and their high-fidelity numerical simulation models
for projection onto the subspace.
While these physics-constrained approaches often
provide stable and accurate predictions with less data,
they require detailed knowledge of the numerical model
and significant development efforts for reduced order model implementation.
\par
Non-intrusive approaches, on the other hand,
attempt to identify the dynamics model purely from data
without requiring knowledge of the underlying physics or high-fidelity simulations.
While the low-dimensional subspace can be identified similar to intrusive approaches,
the model form of latent dynamics vary widely:
simple linear dynamics such as
dynamic mode decomposition (DMD)~\cite{schmid2010dynamic,rowley2009spectral,tu2013dynamic,proctor2016dynamic};
nonlinear dynamics with prescribed model forms
such as operator inference~\cite{peherstorfer2016data,mcquarrie2021data,mcquarrie2023nonintrusive}
and sparse identification of nonlinear dynamics~\cite{brunton2016discovering,fries2022lasdi};
and neural-network-based black-box approaches
such as Neural Operator~\cite{li2020fourier,kovachki2023neural} and DeepONet~\cite{lu2019deeponet}.
Non-intrusive methods typically require more extensive data than intrusive approaches,
but the growing availability of data enables effective training of these models.
\par
The pore collapse and hot spot formation process
presents particular challenges for its reduced order modeling.
The underlying physics is inherently multi-scale, complex and nonlinear,
which in turn requires sophisticated numerical methods for high-fidelity predictions.
This becomes a significant bottleneck for applying intrusive ROM approaches.
Meanwhile, 
computational cost of high-fidelity simulations
and physical limitation in experiments
restrict the generation of extensive training data for non-intrusive ROM approaches.
Several data-driven surrogate modeling methods have been recently proposed
for the shock dynamics of heterogeneous materials~\cite{nguyen2023physics,li2023mapping,springer2023simulating,cheung2024data}.
However, due to limited training data,
the accuracy of instantaneous temperature evoluation is often compromised~\cite{nguyen2023physics},
or predictions are limited to post-shock temperature field~\cite{li2023mapping} or reaction rate~\cite{springer2023simulating}.
Recent work employing DMD for shock-induced pore collapse
successfully predicts instantaneous evolution of temperature field~\cite{cheung2024data}.
However, the linear nature of DMD necessitates training multiple DMD models
for consecutive short time windows,
which reduces the generalizability of the trained model.
\par
Latent dynamics identification (LaSDI)
with greedy sampling~\cite{fries2022lasdi,bonneville2024gplasdi}
is a promising alternative for reduced order modeling of pore collapse process
in data-scarce situation.
LaSDI employs autoencoder to extract essential features of a physics state into a low-dimensional latent space.
The dynamics model for latent variables is expressed as an ordinary differential equation (ODE)
with potential right-hand side terms,
whose coefficients are identified via least-square regression from time series data.
This explicit ODE model form is further assumed to have parametric dependence,
enabling effective interpolative predictions in parameter space.
More importantly,
when equipped with a proper error metric,
this parametric interpolation provides a foundation
for greedy sampling to search for optimal and minimal training samples on the fly.
Such greedy sampling has a great potential for effective latent dynamics learning in data scarce scenarios.
Combining greedy sampling with LaSDI has been explored
with various algorithms for relatively simpler physics systems.
For example, 
k-nearest neighbors convex interpolation
with error metrics based on physics equation residual
has been demonstrated for problems such as Burgers' equation, nonlinear time-dependent heat conduction,
and radial advection problems~\cite{he2023glasdi}.
Gaussian process interpolation has also been applied to more complex physics problems,
such as Vlasov equation and rising thermal bubble phenomena~\cite{bonneville2024gplasdi}.
Gaussian-process-based framework is particularly attractive
because it can quantify the uncertainty of the dynamics under Bayes' law,
which can be used as an error metric even without knowledge of the underlying physics equation.
\par
In this work,
we study the use of Gaussian-process based latent dynamics identification (GPLaSDI)~\cite{bonneville2024gplasdi}
for the pore collapse process.
A shock-induced collapse of a single pore is considered as a simplified testbed
to evaluate the performance of the proposed framework.
\todo{Chris/Keo, can you confirm/add more for the justification of using single pore collapse?}
The trained latent dynamics model could also serve as a fast and accurate subgrid-scale model
in mesoscale predictions.
The key component of the GPLaSDI framework is autoencoder (AE),
which is trained for both latent space extraction and dynamics identification.
While the overall GPLaSDI framework is established,
the autoencoder design is highly problem-specific, depending on the nature of the training data.
This is particularly true for pore collapse dynamics,
where the discontinuous interface between HE and the pore evolves in a complex manner,
including the jetting of HE material.
A naive application of standard AE fails to capture this evolution properly,
thus requiring modifications to its architecture.
In this study,
we present a detailed design process of this autoencoder
in application to the pore collapse dynamics.
\par
The rest of the paper is organized as follows.
Section~\ref{sec:ale3d}
describes the details of the underlying physics model and the training data for pore collapse.
Section~\ref{sec:lasdi} introduces overall framework of GPLaSDI.
Section~\ref{sec:ae} describes the design process and results
for the autoencoder in application to the pore collapse.
Section~\ref{sec:results} presents and discusses
the greedy sampling and prediction result of the trained latent dynamics model.
Finally, conclusions are provided in Section~\ref{sec:conclusion}.


==> sections_lasdi-it.tex <==
\section{The LaSDI-IT Framework}\label{sec:lasdi-it}
\todo[inline]{Kevin: I think we can write this together with section 2.1 to reduce the length and redundancy.}
For a time series of HE temperature field given as $\bT(\bp)$ in (\ref{eq:T}),
the goal is to identify a low-dimensional latent variable $\bz \in \rR^{N_z}$ and its dynamics,
represented as $\dot{\bz} = \cL[\bz; \bp]$,
which can effectively approximate the evolution of the temperature field $\bT(\bp)$.
In this study, we identify the latent dynamics within the framework of GPLaSDI~\cite{bonneville2024gplasdi}.
For a detailed description of the framework,
readers are also referred to prior studies~\cite{fries2022lasdi,bonneville2024gplasdi}.

\subsection{Autoencoder}
\begin{figure*}[tbph]
    \input{figures_schematic.tex}
    \caption{Schematic diagram of latent dynamics identification framework.}
    \label{fig:schematic}
\end{figure*}
Figure~\ref{fig:schematic} illustrates the overall GPLaSDI framework.
First, an autoencoder (AE) is employed to encapsulate essential features of a temperature field $T(\bp)$
onto a low-dimensional nonlinear manifold.
Typically, an AE consists of two neural-networks (NNs): an encoder and a decoder,
\begin{subequations}
    \begin{equation}\label{eq:en}
    \bz = \En(T;\theta_{en})
    \end{equation}
    \begin{equation}\label{eq:de}
    T = \De(\bz;\theta_{de}),
    \end{equation}
\end{subequations}
with their weight and biases denoted as $\theta_{en}$ and $\theta_{de}$.
The encoder compresses the high-dimensional temperature field into a latent space variable $\bz$,
while the decoder reconstructs the temperature field from the latent space variable.
\par
To effectively train an autoencoder,
scaling of the training data is often required.
This is particularly true for pore collapse problems,
where drastic change in temperature occurs in a localized region near the pore during the hot spot development.
To ensure uniform variance in temperature across the grid space,
the temperature field is scaled with temporal average $\overline{T}$ and standard deviation $\std[T]$,
\begin{equation}\label{eq:T-scale}
\tT = \frac{T - \overline{T}}{\std[T]},
\end{equation}
where $\overline{T}$ and $\std[T]$ are evaluated over the entire training data $\rT$,
\begin{subequations}\label{eq:T-scale0}
\begin{equation}
\overline{T} = \frac{1}{N_pN_t}\sum_{p}^{N_p}\sum_k^{N_t}T_k(\bp_p)
\end{equation}
\begin{equation}
\std[T] =
\left(
    \frac{1}{N_pN_t}\sum_{p}^{N_p}\sum_k^{N_t}T_k^2(\bp_p) - \overline{T}^2
\right)^{1/2}.
\end{equation}    
\end{subequations}
This scaling helps the autoencoder learn the features of temperature field uniformly across the grid points.
\par
The NN parameters are trained to minimize the reconstruction loss of (scaled) training data,
\begin{equation}\label{eq:J-ae0}
\cJ_{AE} = \frac{1}{N_pN_tN_x}\sum_p^{N_p}\sum_k^{N_t}
\Vert \tT_k(\bp_p) - \De(\En(\tT_k(\bp_p); \theta_{en}); \theta_{de}) \Vert^2.
\end{equation}
With scaling with temporal average and standard deviation (\ref{eq:T-scale0}),
the reconstruction loss (\ref{eq:J-ae0}) of an untrained AE is typically $\cJ_{AE}\sim\cO(1)$.
An effective AE---that can reconstruct $T$ from much lower dimensional $\bz$ with shorter training time---is
a key for identifying accurate latent space dynamics.
Designing AE is highly problem-specific and must account for the nature of the given data.
This, in turn, also involves revision of the scaling (\ref{eq:T-scale0}) and the loss definition (\ref{eq:J-ae0}).
The specific architecture, loss term and its designing process for pore collapse will be described in Section~\ref{sec:ae}.

\subsection{Latent dynamics identification}
The evolution of the latent space variable $\bz$, as captured by AE,
is represented using sparse identification of nonlinear dynamics (SINDy)~\cite{brunton2016discovering,fries2022lasdi}.
The evolution of $\bz$ is expressed as a system of ordinary differential equations (ODEs)
with a right-hand side composed of candidate terms,
\begin{equation}\label{eq:lasdi}
\dot{\bz} = \bXi(\bp)^{\top}\bPhi(\bz)^{\top},
\end{equation}
with $\bPhi$ a dictionary for candidate terms and $\bXi$ their corresponding coefficients.
For example of a general quadratic ODE system,
\begin{equation}
\bPhi(\bz) =
\begin{pmatrix}
1 & \bz^{\top} & z_1^2 & z_2^2 & \ldots & z_1z_2 & \ldots & z_{N_t-1}z_{N_t}
\end{pmatrix}.
\end{equation}
While SINDy allows general nonlinear terms,
we limit the latnet dynamics to be only a linear dynamics for pore collapse problem.
This choice is motivated by two factors.
First, 
limiting to linear dynamics significantly reduces the number of coefficients to be fitted,
decreasing the risk of overfitting without sparse regression.
This allows us to prevent a potential slow-down in multi-objective training with an additional sparsity regularization term.
Second,
while the temperature field exhibits complex features,
its evolution is predominantly one-directional as the shock propagates through the domain.
Once the shock passes and the pore fully collapses,
the temperature field reaches a quasi-steady state.
This observation leads to an expectation that the evolution of the temperature field
can be sufficiently represented by linear dynamics with a single fixed point
with the autoencoder capturing the nonlinear solution manifold.
%while the complex nonlinear solution manifold is captured by an autoencoder.
\par
The coefficients of the linear latent dynamics are estimated from data using linear regression.
From a time series of temperature field $\bT(\bp)$,
we obtain the time series of corresponding latent variables encoded by AE,
\begin{equation}
\bZ \equiv \En(\bT) =
\begin{pmatrix}
\bz_1 & \bz_2 & \ldots & \bz_{N_t}
\end{pmatrix}
\in\rR^{N_z\times N_t}.
\end{equation}
The time derivative of this data $\bZ$ is evaluated using finite-difference (FD) approximation,
\begin{equation}
\dot{\bZ}
\approx
\frac{1}{\Delta t}\bZ\bD_t^{\top},
\end{equation}
where $\Delta t=10^{-2}ns$ and $\bD_t\in\rR^{N_t\times N_t}$ is a FD stencil operator using summation-by-part 2nd-4th order stencil~\cite{kreiss1974finite,hicken2013summation}.
Given $\bZ$ and $\dot{\bZ}$,
we seek the coefficient $\bXi\in\rR^{(N_z+1)\times N_z}$ that best-minimizes the residual for the governing ODE system,
\begin{equation}
\bXi = \arg\min\limits_{\tilde{\bXi}} \left\Vert \frac{1}{\Delta t}\bD_t\bZ^{\top} - \bPhi(\bZ)\tilde{\bXi} \right\Vert^2,
\end{equation}
with the candidate right-hand side term for training data
\begin{equation}
\bPhi(\bZ) = 
\begin{pmatrix}
\mathbf{1} & \bZ^{\top}
\end{pmatrix}
\in \rR^{N_t\times (N_z+1)}.
\end{equation}
This minimizer can be obtained using the pseudo-inverse of $\bPhi$,
\begin{equation}\label{eq:xi}
\bXi(\bp) = \frac{1}{\Delta t}\bPhi(\bZ(\bp))^{\dagger}\bD_t\bZ(\bp)^{\top}.
\end{equation}
\par
In the GPLaSDI framework, the autoencoder is trained to minimize the remaining residual of latent dynamics as well,
\begin{equation}\label{eq:J-ld}
\cJ_{LD} = \frac{1}{N_p}\sum_p^{N_p}\left\Vert \frac{1}{\Delta t}\bD_t\bZ(\bp_p)^{\top} - \bPhi(\bZ(\bp_p))\bXi(\bp_p) \right\Vert^2,
\end{equation}
where the minimizer (\ref{eq:xi}) is plugged into the ODE residual.
The reconstruction loss $\cJ_{AE}$ and the remaining latent dynamics residual $\cJ_{LD}$
are jointly trained using a single loss function,
\begin{equation}\label{eq:J}
\cJ = \cJ_{AE} + \beta_1\cJ_{LD}.
\end{equation}
While Bonneville \textit{et al.}~\cite{bonneville2024gplasdi} also included a $L_2$-norm regularization term for the coefficient $\bXi$,
such regularization was not needed for the pore collapse problem.
Also, optimal value for the relative weight $\beta_1$ is entirely problem-specific and requires hyper-parameter tuning,
though we recommend tuning it in unit of $\Delta t^2$.
The rationale is that, with (\ref{eq:xi}),
the latent dynamics loss (\ref{eq:J-ld}) is always multiplied by a factor of $\Delta t^{-2}$.
Thus, this approach essentially non-dimensionalizes $\cJ_{LD}$ regardless of the unit of $\Delta t$,
reducing the effort in hyper-parameter tuning.
Throughout this study, $\beta_1 = 10^2\Delta t^2$ is used.
The autoencoder is trained for (\ref{eq:J}) using Adam optimizer throughout this study~\cite{kingma2014adam}.

\subsection{Parametric interpolation and greedy sampling via Gaussian-process}
Once the dynamics coefficients $\bXi$ are identified for the training parameter points
$\{\bp_1, \bp_2, \ldots, \bp_{N_t}\}$,
the next step is to estimate the coefficients at unseen parameter point, i.e. $\bXi(\bp^*)$,
based on the `measurements' $\cD=\{\bXi(\bp_1), \bXi(\bp_2), \ldots, \bXi(\bp_{N_t})\}$.
Gaussian process (GP) is employed for this purpose~\cite{rasmussen2003gaussian}.
For an entry of the coefficient matrix, $\Xi_{ij}$,
the measurement data $\cD_{ij}=\{\Xi_{ij}(\bp_1), \ldots, \Xi_{ij}(\bp_{N_p})\}\in\rR^{N_p}$
is given at the training parameter points $\rP$.
Each $\Xi_{ij}$ is treated as an uncertain variable that follows an independent Gaussian process,
\begin{equation}\label{eq:gp}
\Xi_{ij}(\bp)
\sim
\GP\!\left[\overline{\Xi}_{ij}(\bp), K(\bp, \bp')\right]
+
\epsilon.
\end{equation}
The GP assumes a prior mean model $\overline{\Xi}_{ij}(\bp): \rR^{N_p}\to \rR$
and uses a covariance kernel $K(\bp, \bp'): \rR^{N_p}\times\rR^{N_p}\to \rR$
to quantify the relationship between parameter points.
Additionally, the `observation' Gaussian noise $\epsilon\sim\cN(0, \sigma^2)$
is incorporated into the GP model,
though it is used only for optimization stability with a negligibly small value $\sigma=10^{-6}$.
Without any prior knowledge, the prior mean model is assumed to be zero,
i.e. $\overline{\Xi}_{ij}(\bp)=0$.
The covariance kernel is defined using radial basis function (RBF) over the parameter space,
\begin{equation}
K(\bp, \bp'; \theta_{GP})
=
\gamma
\exp\left( - \frac{\Vert \bp - \bp'\Vert^2}{2\lambda^2} \right),
\end{equation}
where the variance $\gamma\in\rR^+$ and the correlation scale $\lambda\in\rR^+$
are the hyperparameter $\theta_{GP}=\{\gamma, \lambda\}$ to be calibrated.
For two sets of parameter points
$\rP_I=\{\bp_1,\ldots,\bp_{N_i}\}$ and $\rP_J=\{\bp_1,\ldots,\bp_{N_j}\}$,
the covariance matrix $\bK(\rP_I, \rP_J)\in \rR^{N_p\times N_p}$ is defined,
\begin{equation}
(\bK)_{ij} = K(\bp_i, \bp_j;\theta_{GP})
\quad
\bp_i\in\rP_I
\quad
\bp_j\in\rP_J.
\end{equation}
\par
The hyperparameter $\theta_{GP}=\{\gamma, \lambda\}$ is calibrated
to maximize the likelihood of the measurement data $\cD_{ij}$
at the training parameter points $\rP$.
Per GP model (\ref{eq:gp}), the likelihood of the measurement data
follows a joint normal distribution,
\begin{equation}\label{eq:marginal-likelihood}
P(\cD_{ij} | \theta_{GP})
\sim
\cN[0, \bK(\rP, \rP) + \sigma^2\mathbf{I}_{N_p}].
\end{equation}
$\theta_{GP}=\{\gamma, \lambda\}$ is then calibrated to be the maximizer of (\ref{eq:marginal-likelihood}).
Throughout this study, the calibration of $\theta_{GP}$ is performed with the python \texttt{scikit} package~\cite{scikit-learn}.
\par
Conditioned upon the data $\cD_{ij}$,
the probability of the coefficient at unseen parameter point, i.e. $\Xi_{ij}(\bp^*)$,
also follows a normal distribution~\cite{rasmussen2003gaussian},
\begin{subequations}\label{eq:gp-predict}
\begin{equation}
P(\Xi_{ij}(\bp^*) | \cD_{ij}, \theta_{GP})
\sim
\cN[\tilde{\Xi}_{ij}(\bp^*), \mathrm{Var}(\Xi_{ij}(\bp^*))],
\end{equation}
where the conditional average and variance are given as
\begin{equation}\label{eq:gp-cond-avg}
\tilde{\Xi}_{ij}(\bp^*) = \bK(\bp^*, \rP)(\bK(\rP, \rP) + \sigma^2\mathbf{I}_{N_p})^{-1}\cD_{ij}
\end{equation}
\begin{equation}\label{eq:gp-cond-var}
\begin{split}
&\mathrm{Var}(\Xi_{ij}(\bp^*)) = \bK(\bp^*, \bp^*)\\
&\qquad - \bK(\bp^*, \rP)(\bK(\rP, \rP) + \sigma^2\mathbf{I}_{N_p})^{-1}\bK(\rP, \bp^*).
\end{split}
\end{equation}
\end{subequations}
\par
A prediction at unseen parameter point $\bp^*$ would involve
either using the conditional average (\ref{eq:gp-cond-avg})
or sampling from the probability (\ref{eq:gp-predict})
for all coefficients, to construct the dynamics coefficients $\bXi(\bp^*)$.
The estimated $\bXi(\bp^*)$ is then used to simulate the latent dynamics (\ref{eq:lasdi}),
with initial condition $\bz_0(\bp^*) = \En(\bT(\bp^*))$
encoded from the initial temperature field for the parameter point $\bp^*$.
The latent space trajectory $\{\bz_1, \ldots, \bz_{N_t}\}$ is then
decoded back to the temperature field for prediction.
The overall framework is also illustrated in Figure~\ref{fig:schematic}.
\par
If initial training data is scarce in parameter space
and not sufficient for effective parametric model training,
data at additional parameter points must be collected on the fly
in the training process.
Gaussian process also provides the uncertainties in the dynamics coefficients,
which are useful error metrics in the absence of ground truth.
In GPLaSDI framework,
The uncertainties of $\bXi(\bp^*)$ (\ref{eq:gp-predict})
are forward propagated toward the temperature field $\bT$
at candidate sampling points $\bp^*_1, \bp^*_2, \ldots, \bp^*_{N_p^*}$,
via Monte-Carlo sampling.
First, at each parameter point $\bp^*_i$,
$N_s$ samples of $\{\bXi_s(\bp^*_i)\}_{s=1}^{N_s}$ are collected from the probability distribution (\ref{eq:gp-predict}).
Samples of temperature field
% i.e. $\rT_{gp}(\bp^*_i) = \{\bT^1(\bp^*_i), \bT^2(\bp^*_i), \ldots, \bT^{N_s}(\bp^*_i)\}$,
are then collected from the simulations of the latent dynamics (\ref{eq:lasdi}) with the samples of $\bXi(\bp^*_i)$.
We denote this sample temperature field tensor as $\rT_{gp}\in\rR^{N_p^*\times N_t \times N_x \times N_s}$,
where $(\rT_{gp})_{ijkl} = \rT_{gp}(\bp^*_i, t_j, \bx_k, \bXi_l)$ represents
the HE temperature at grid point $\bx_k$, time $t_j$ for parameter $\bp^*_i$, predicted with the sample coefficients $\bXi_l$.
From $\rT_{gp}$, the solution uncertainty is evaluated with
the standard deviation of the sample temperature fields,
\begin{subequations}\label{eq:uq-metric}
\begin{equation}
\begin{split}
&\std_{gp}[\rT_{gp}](\bp^*_i) = \\
&\max_{t_j}
\frac{1}{N_x}\sum_{k=1}^{N_x}
\frac{1}{N_s}\sum_{s=1}^{N_s}
\{ \rT_{gp}(\bp^*_i, t_j, \bx_k, \bXi_s) - \overline{\rT}_{gp}(\bp^*_i, t_j, \bx_k) \}^2,
\end{split}
\end{equation}
where $\overline{\rT}_{gp}$ is the sample average of $\rT_{gp}$,
\begin{equation}
\overline{\rT}_{gp}(\bp^*_i, t_j, \bx_k) = \frac{1}{N_s}\sum_{s=1}^{N_s}\rT_{gp}(\bp^*_i, t_j, \bx_k, \bXi_s) \in \rR^{N_p^* \times N_x\times N_t}.
\end{equation}
\end{subequations}
The parameter point with the maximum uncertainty (\ref{eq:uq-metric}) is picked up as a new training parameter point,
\begin{equation}\label{eq:next-p}
\bp_{N_p+1} = \arg\max_i\;\std_{gp}[\rT_{gp}](\bp^*_i).
\end{equation}
The corresponding full-order model solution is then collected
and appended to the existing training data for the on-going training,
\begin{equation}
\rT = \{\bT(\bp_1), \bT(\bp_2), \ldots, \bT(\bp_{N_p}), \bT(\bp_{N_p+1})\}.
\end{equation}
The temporal average and standard deviation in (\ref{eq:T-scale0}) are updated accordingly.
We also refer readers to Bonneville \textit{et al.}~\cite{bonneville2024gplasdi} for the detailed algorithm of this greedy sampling process.
\par
Note that, unlike Bonneville \textit{et al.}~\cite{bonneville2024gplasdi}
who maximize over both space and time for the sample standard deviation,
we averaged the sample standard deviation over space as uncertainty metric.
Considering the temperature field data shown in Figure~\ref{fig:he-temp},
sample variance for masking pore region causes high-temperature standard deviation near the discontinuous pore interface.
Maximum sample standard deviation will be always chosen from the pore interface region,
thus not appropriately representing the uncertainty of the overall solution.
For this reason, we evaluate the sample standard deviation to be averaged over space.


==> sections_lasdi.tex <==
\section{Overall framework}\label{sec:lasdi}
For a time series of HE temperature field given as $\bT(\bp)$ in (\ref{eq:T}),
the goal is to identify a low-dimensional latent variable $\bz \in \rR^{N_z}$ and its dynamics,
represented as $\dot{\bz} = \cL[\bz; \bp]$,
which can effectively approximate the evolution of the temperature field $\bT(\bp)$.
In this study, we identify the latent dynamics within the framework of GPLaSDI~\cite{bonneville2024gplasdi}.
For a detailed description of the framework,
readers are also referred to prior studies~\cite{fries2022lasdi,bonneville2024gplasdi}.

\subsection{Autoencoder}
\begin{figure*}[tbph]
    \input{figures_schematic.tex}
    \caption{Schematic diagram of latent dynamics identification framework.}
    \label{fig:schematic}
\end{figure*}
Figure~\ref{fig:schematic} illustrates the overall GPLaSDI framework.
First, an autoencoder (AE) is employed to encapsulate essential features of a temperature field $T(\bp)$
onto a low-dimensional nonlinear manifold.
Typically, an AE consists of two neural-networks (NNs): an encoder and a decoder,
\begin{subequations}
    \begin{equation}\label{eq:en}
    \bz = \En(T;\theta_{en})
    \end{equation}
    \begin{equation}\label{eq:de}
    T = \De(\bz;\theta_{de}),
    \end{equation}
\end{subequations}
with their weight and biases denoted as $\theta_{en}$ and $\theta_{de}$.
The encoder compresses the high-dimensional temperature field into a latent space variable $\bz$,
while the decoder reconstructs the temperature field from the latent space variable.
\par
To effectively train an autoencoder,
scaling of the training data is often required.
This is particularly true for pore collapse problems,
where drastic change in temperature occurs in a localized region near the pore during the hot spot development.
To ensure uniform variance in temperature across the grid space,
the temperature field is scaled with temporal average $\overline{T}$ and standard deviation $\std[T]$,
\begin{equation}\label{eq:T-scale}
\tT = \frac{T - \overline{T}}{\std[T]},
\end{equation}
where $\overline{T}$ and $\std[T]$ are evaluated over the entire training data $\rT$,
\begin{subequations}\label{eq:T-scale0}
\begin{equation}
\overline{T} = \frac{1}{N_pN_t}\sum_{p}^{N_p}\sum_k^{N_t}T_k(\bp_p)
\end{equation}
\begin{equation}
\std[T] =
\left(
    \frac{1}{N_pN_t}\sum_{p}^{N_p}\sum_k^{N_t}T_k^2(\bp_p) - \overline{T}^2
\right)^{1/2}.
\end{equation}    
\end{subequations}
This scaling helps the autoencoder learn the features of temperature field uniformly across the grid points.
\par
The NN parameters are trained to minimize the reconstruction loss of (scaled) training data,
\begin{equation}\label{eq:J-ae0}
\cJ_{AE} = \frac{1}{N_pN_tN_x}\sum_p^{N_p}\sum_k^{N_t}
\Vert \tT_k(\bp_p) - \De(\En(\tT_k(\bp_p); \theta_{en}); \theta_{de}) \Vert^2.
\end{equation}
With scaling with temporal average and standard deviation (\ref{eq:T-scale0}),
the reconstruction loss (\ref{eq:J-ae0}) of an untrained AE is typically $\cJ_{AE}\sim\cO(1)$.
An effective AE---that can reconstruct $T$ from much lower dimensional $\bz$ with shorter training time---is
a key for identifying accurate latent space dynamics.
Designing AE is highly problem-specific and must account for the nature of the given data.
This, in turn, also involves revision of the scaling (\ref{eq:T-scale0}) and the loss definition (\ref{eq:J-ae0}).
The specific architecture, loss term and its designing process for pore collapse will be described in Section~\ref{sec:ae}.

\subsection{Latent dynamics identification}
The evolution of the latent space variable $\bz$, as captured by AE,
is represented using sparse identification of nonlinear dynamics (SINDy)~\cite{brunton2016discovering,fries2022lasdi}.
The evolution of $\bz$ is expressed as a system of ordinary differential equations (ODEs)
with a right-hand side composed of candidate terms,
\begin{equation}\label{eq:lasdi}
\dot{\bz} = \bXi(\bp)^{\top}\bPhi(\bz)^{\top},
\end{equation}
with $\bPhi$ a dictionary for candidate terms and $\bXi$ their corresponding coefficients.
For example of a general quadratic ODE system,
\begin{equation}
\bPhi(\bz) =
\begin{pmatrix}
1 & \bz^{\top} & z_1^2 & z_2^2 & \ldots & z_1z_2 & \ldots & z_{N_t-1}z_{N_t}
\end{pmatrix}.
\end{equation}
While SINDy allows general nonlinear terms,
we limit the latnet dynamics to be only a linear dynamics for pore collapse problem.
This choice is motivated by two factors.
First, 
limiting to linear dynamics significantly reduces the number of coefficients to be fitted,
decreasing the risk of overfitting without sparse regression.
This allows us to prevent a potential slow-down in multi-objective training with an additional sparsity regularization term.
Second,
while the temperature field exhibits complex features,
its evolution is predominantly one-directional as the shock propagates through the domain.
Once the shock passes and the pore fully collapses,
the temperature field reaches a quasi-steady state.
This observation leads to an expectation that the evolution of the temperature field
can be sufficiently represented by linear dynamics with a single fixed point
with the autoencoder capturing the nonlinear solution manifold.
%while the complex nonlinear solution manifold is captured by an autoencoder.
\par
The coefficients of the linear latent dynamics are estimated from data using linear regression.
From a time series of temperature field $\bT(\bp)$,
we obtain the time series of corresponding latent variables encoded by AE,
\begin{equation}
\bZ \equiv \En(\bT) =
\begin{pmatrix}
\bz_1 & \bz_2 & \ldots & \bz_{N_t}
\end{pmatrix}
\in\rR^{N_z\times N_t}.
\end{equation}
The time derivative of this data $\bZ$ is evaluated using finite-difference (FD) approximation,
\begin{equation}
\dot{\bZ}
\approx
\frac{1}{\Delta t}\bZ\bD_t^{\top},
\end{equation}
where $\Delta t=10^{-2}ns$ and $\bD_t\in\rR^{N_t\times N_t}$ is a FD stencil operator using summation-by-part 2nd-4th order stencil~\cite{kreiss1974finite,hicken2013summation}.
Given $\bZ$ and $\dot{\bZ}$,
we seek the coefficient $\bXi\in\rR^{(N_z+1)\times N_z}$ that best-minimizes the residual for the governing ODE system,
\begin{equation}
\bXi = \arg\min\limits_{\tilde{\bXi}} \left\Vert \frac{1}{\Delta t}\bD_t\bZ^{\top} - \bPhi(\bZ)\tilde{\bXi} \right\Vert^2,
\end{equation}
with the candidate right-hand side term for training data
\begin{equation}
\bPhi(\bZ) = 
\begin{pmatrix}
\mathbf{1} & \bZ^{\top}
\end{pmatrix}
\in \rR^{N_t\times (N_z+1)}.
\end{equation}
This minimizer can be obtained using the pseudo-inverse of $\bPhi$,
\begin{equation}\label{eq:xi}
\bXi(\bp) = \frac{1}{\Delta t}\bPhi(\bZ(\bp))^{\dagger}\bD_t\bZ(\bp)^{\top}.
\end{equation}
\par
In the GPLaSDI framework, the autoencoder is trained to minimize the remaining residual of latent dynamics as well,
\begin{equation}\label{eq:J-ld}
\cJ_{LD} = \frac{1}{N_p}\sum_p^{N_p}\left\Vert \frac{1}{\Delta t}\bD_t\bZ(\bp_p)^{\top} - \bPhi(\bZ(\bp_p))\bXi(\bp_p) \right\Vert^2,
\end{equation}
where the minimizer (\ref{eq:xi}) is plugged into the ODE residual.
The reconstruction loss $\cJ_{AE}$ and the remaining latent dynamics residual $\cJ_{LD}$
are jointly trained using a single loss function,
\begin{equation}\label{eq:J}
\cJ = \cJ_{AE} + \beta_1\cJ_{LD}.
\end{equation}
While Bonneville \textit{et al.}~\cite{bonneville2024gplasdi} also included a $L_2$-norm regularization term for the coefficient $\bXi$,
such regularization was not needed for the pore collapse problem.
Also, optimal value for the relative weight $\beta_1$ is entirely problem-specific and requires hyper-parameter tuning,
though we recommend tuning it in unit of $\Delta t^2$.
The rationale is that, with (\ref{eq:xi}),
the latent dynamics loss (\ref{eq:J-ld}) is always multiplied by a factor of $\Delta t^{-2}$.
Thus, this approach essentially non-dimensionalizes $\cJ_{LD}$ regardless of the unit of $\Delta t$,
reducing the effort in hyper-parameter tuning.
Throughout this study, $\beta_1 = 10^2\Delta t^2$ is used.
The autoencoder is trained for (\ref{eq:J}) using Adam optimizer throughout this study~\cite{kingma2014adam}.

\subsection{Parametric interpolation and greedy sampling via Gaussian-process}
Once the dynamics coefficients $\bXi$ are identified for the training parameter points
$\{\bp_1, \bp_2, \ldots, \bp_{N_t}\}$,
the next step is to estimate the coefficients at unseen parameter point, i.e. $\bXi(\bp^*)$,
based on the `measurements' $\cD=\{\bXi(\bp_1), \bXi(\bp_2), \ldots, \bXi(\bp_{N_t})\}$.
Gaussian process (GP) is employed for this purpose~\cite{rasmussen2003gaussian}.
For an entry of the coefficient matrix, $\Xi_{ij}$,
the measurement data $\cD_{ij}=\{\Xi_{ij}(\bp_1), \ldots, \Xi_{ij}(\bp_{N_p})\}\in\rR^{N_p}$
is given at the training parameter points $\rP$.
Each $\Xi_{ij}$ is treated as an uncertain variable that follows an independent Gaussian process,
\begin{equation}\label{eq:gp}
\Xi_{ij}(\bp)
\sim
\GP\!\left[\overline{\Xi}_{ij}(\bp), K(\bp, \bp')\right]
+
\epsilon.
\end{equation}
The GP assumes a prior mean model $\overline{\Xi}_{ij}(\bp): \rR^{N_p}\to \rR$
and uses a covariance kernel $K(\bp, \bp'): \rR^{N_p}\times\rR^{N_p}\to \rR$
to quantify the relationship between parameter points.
Additionally, the `observation' Gaussian noise $\epsilon\sim\cN(0, \sigma^2)$
is incorporated into the GP model,
though it is used only for optimization stability with a negligibly small value $\sigma=10^{-6}$.
Without any prior knowledge, the prior mean model is assumed to be zero,
i.e. $\overline{\Xi}_{ij}(\bp)=0$.
The covariance kernel is defined using radial basis function (RBF) over the parameter space,
\begin{equation}
K(\bp, \bp'; \theta_{GP})
=
\gamma
\exp\left( - \frac{\Vert \bp - \bp'\Vert^2}{2\lambda^2} \right),
\end{equation}
where the variance $\gamma\in\rR^+$ and the correlation scale $\lambda\in\rR^+$
are the hyperparameter $\theta_{GP}=\{\gamma, \lambda\}$ to be calibrated.
For two sets of parameter points
$\rP_I=\{\bp_1,\ldots,\bp_{N_i}\}$ and $\rP_J=\{\bp_1,\ldots,\bp_{N_j}\}$,
the covariance matrix $\bK(\rP_I, \rP_J)\in \rR^{N_p\times N_p}$ is defined,
\begin{equation}
(\bK)_{ij} = K(\bp_i, \bp_j;\theta_{GP})
\quad
\bp_i\in\rP_I
\quad
\bp_j\in\rP_J.
\end{equation}
\par
The hyperparameter $\theta_{GP}=\{\gamma, \lambda\}$ is calibrated
to maximize the likelihood of the measurement data $\cD_{ij}$
at the training parameter points $\rP$.
Per GP model (\ref{eq:gp}), the likelihood of the measurement data
follows a joint normal distribution,
\begin{equation}\label{eq:marginal-likelihood}
P(\cD_{ij} | \theta_{GP})
\sim
\cN[0, \bK(\rP, \rP) + \sigma^2\mathbf{I}_{N_p}].
\end{equation}
$\theta_{GP}=\{\gamma, \lambda\}$ is then calibrated to be the maximizer of (\ref{eq:marginal-likelihood}).
Throughout this study, the calibration of $\theta_{GP}$ is performed with the python \texttt{scikit} package~\cite{scikit-learn}.
\par
Conditioned upon the data $\cD_{ij}$,
the probability of the coefficient at unseen parameter point, i.e. $\Xi_{ij}(\bp^*)$,
also follows a normal distribution~\cite{rasmussen2003gaussian},
\begin{subequations}\label{eq:gp-predict}
\begin{equation}
P(\Xi_{ij}(\bp^*) | \cD_{ij}, \theta_{GP})
\sim
\cN[\tilde{\Xi}_{ij}(\bp^*), \mathrm{Var}(\Xi_{ij}(\bp^*))],
\end{equation}
where the conditional average and variance are given as
\begin{equation}\label{eq:gp-cond-avg}
\tilde{\Xi}_{ij}(\bp^*) = \bK(\bp^*, \rP)(\bK(\rP, \rP) + \sigma^2\mathbf{I}_{N_p})^{-1}\cD_{ij}
\end{equation}
\begin{equation}\label{eq:gp-cond-var}
\begin{split}
&\mathrm{Var}(\Xi_{ij}(\bp^*)) = \bK(\bp^*, \bp^*)\\
&\qquad - \bK(\bp^*, \rP)(\bK(\rP, \rP) + \sigma^2\mathbf{I}_{N_p})^{-1}\bK(\rP, \bp^*).
\end{split}
\end{equation}
\end{subequations}
\par
A prediction at unseen parameter point $\bp^*$ would involve
either using the conditional average (\ref{eq:gp-cond-avg})
or sampling from the probability (\ref{eq:gp-predict})
for all coefficients, to construct the dynamics coefficients $\bXi(\bp^*)$.
The estimated $\bXi(\bp^*)$ is then used to simulate the latent dynamics (\ref{eq:lasdi}),
with initial condition $\bz_0(\bp^*) = \En(\bT(\bp^*))$
encoded from the initial temperature field for the parameter point $\bp^*$.
The latent space trajectory $\{\bz_1, \ldots, \bz_{N_t}\}$ is then
decoded back to the temperature field for prediction.
The overall framework is also illustrated in Figure~\ref{fig:schematic}.
\par
If initial training data is scarce in parameter space
and not sufficient for effective parametric model training,
data at additional parameter points must be collected on the fly
in the training process.
Gaussian process also provides the uncertainties in the dynamics coefficients,
which are useful error metrics in the absence of ground truth.
In GPLaSDI framework,
The uncertainties of $\bXi(\bp^*)$ (\ref{eq:gp-predict})
are forward propagated toward the temperature field $\bT$
at candidate sampling points $\bp^*_1, \bp^*_2, \ldots, \bp^*_{N_p^*}$,
via Monte-Carlo sampling.
First, at each parameter point $\bp^*_i$,
$N_s$ samples of $\{\bXi_s(\bp^*_i)\}_{s=1}^{N_s}$ are collected from the probability distribution (\ref{eq:gp-predict}).
Samples of temperature field
% i.e. $\rT_{gp}(\bp^*_i) = \{\bT^1(\bp^*_i), \bT^2(\bp^*_i), \ldots, \bT^{N_s}(\bp^*_i)\}$,
are then collected from the simulations of the latent dynamics (\ref{eq:lasdi}) with the samples of $\bXi(\bp^*_i)$.
We denote this sample temperature field tensor as $\rT_{gp}\in\rR^{N_p^*\times N_t \times N_x \times N_s}$,
where $(\rT_{gp})_{ijkl} = \rT_{gp}(\bp^*_i, t_j, \bx_k, \bXi_l)$ represents
the HE temperature at grid point $\bx_k$, time $t_j$ for parameter $\bp^*_i$, predicted with the sample coefficients $\bXi_l$.
From $\rT_{gp}$, the solution uncertainty is evaluated with
the standard deviation of the sample temperature fields,
\begin{subequations}\label{eq:uq-metric}
\begin{equation}
\begin{split}
&\std_{gp}[\rT_{gp}](\bp^*_i) = \\
&\max_{t_j}
\frac{1}{N_x}\sum_{k=1}^{N_x}
\frac{1}{N_s}\sum_{s=1}^{N_s}
\{ \rT_{gp}(\bp^*_i, t_j, \bx_k, \bXi_s) - \overline{\rT}_{gp}(\bp^*_i, t_j, \bx_k) \}^2,
\end{split}
\end{equation}
where $\overline{\rT}_{gp}$ is the sample average of $\rT_{gp}$,
\begin{equation}
\overline{\rT}_{gp}(\bp^*_i, t_j, \bx_k) = \frac{1}{N_s}\sum_{s=1}^{N_s}\rT_{gp}(\bp^*_i, t_j, \bx_k, \bXi_s) \in \rR^{N_p^* \times N_x\times N_t}.
\end{equation}
\end{subequations}
The parameter point with the maximum uncertainty (\ref{eq:uq-metric}) is picked up as a new training parameter point,
\begin{equation}\label{eq:next-p}
\bp_{N_p+1} = \arg\max_i\;\std_{gp}[\rT_{gp}](\bp^*_i).
\end{equation}
The corresponding full-order model solution is then collected
and appended to the existing training data for the on-going training,
\begin{equation}
\rT = \{\bT(\bp_1), \bT(\bp_2), \ldots, \bT(\bp_{N_p}), \bT(\bp_{N_p+1})\}.
\end{equation}
The temporal average and standard deviation in (\ref{eq:T-scale0}) are updated accordingly.
We also refer readers to Bonneville \textit{et al.}~\cite{bonneville2024gplasdi} for the detailed algorithm of this greedy sampling process.
\par
Note that, unlike Bonneville \textit{et al.}~\cite{bonneville2024gplasdi}
who maximize over both space and time for the sample standard deviation,
we averaged the sample standard deviation over space as uncertainty metric.
Considering the temperature field data shown in Figure~\ref{fig:he-temp},
sample variance for masking pore region causes high-temperature standard deviation near the discontinuous pore interface.
Maximum sample standard deviation will be always chosen from the pore interface region,
thus not appropriately representing the uncertainty of the overall solution.
For this reason, we evaluate the sample standard deviation to be averaged over space.


==> sections_results.tex <==
\section{Results}\label{sec:results}
The GPLaSDI framework in Section~\ref{sec:lasdi},
combined with the revised autoencoder in Section~\ref{sec:ae},
is applied to identify latent dynamics of single pore collapse processes.
For physics parameters,
the angle $p_1$ and the length $p_2$ of the major axis of the pore are considered
for ranges of $\bp = (p_1, p_2) \in [\deg{0}, \deg{20}]\times [1\mu m, 1.2\mu m]$.
This section demonstrates the effectiveness of the GPLaSDI framework, particularly in data-scarce scenarios.
\par
To simulate a data-scarce situation,
the initial training dataset consisted of only four parameter points
located at the corners of the parameter space:
$\rP^{(0)} = \{(\deg{0}, 1\mu m), (\deg{20}, 1\mu m), (\deg{0}, 1.2\mu m), (\deg{20}, 1.2\mu m)\}$.
For an inner-loop training,
the revised autoencoder is trained on the available training data
to minimize the objective (\ref{eq:J}) with $\beta_1 = 10^2\Delta t^2$,
where $\cJ_{AE}$ and $\cJ_{LD}$ are defined in (\ref{eq:J-ae1}) and (\ref{eq:J-ld}), respectively.
Each inner-loop training took $2000$ iterations of ADAM optimization
with a learning rate of $10^{-4}$.
At the end of each inner loop,
the conditional probability of the coefficients (\ref{eq:gp-predict})
is evaluated over 121 test points of parameter space.
The test points are chosen to be a $11\times11$ array
uniformly distributed on $[\deg{0}, \deg{20}]\times [1\mu m, 1.2\mu m]$.
This dynamics uncertainty is then forward-propagated
to the solution uncertainty (\ref{eq:uq-metric}) with 30 Monte Carlo samples at each test point.
Based on the solution uncertainty, the next training parameter point was selected
using the greedy sampling criterion (\ref{eq:next-p}).
This new parameter point was added to the training dataset,
and the outer-loop process was repeated with gradually increasing training data.
\par
\begin{figure}[tbph]
    \input{figures_gp_uncertainty.tex}
    \caption{Gaussian-process based coefficient interpolation at the 14th iteration:
    (a) Mean and (b) standard deviation of the coefficient $\Xi_{15}$.
    White markers indicate the sampled training data.}
    \label{fig:gp-uncertainty}
\end{figure}
Figure~\ref{fig:gp-uncertainty} shows the average (\ref{eq:gp-cond-avg})
and the standard deviation (square-root of \ref{eq:gp-cond-var})
of the dynamics coefficient $\Xi_{15}$,
conditioned upon the training data at the 14th outer loop iteration.
Overall, the mean coefficient exhibits smooth variation across the parameter space,
indicating that the GP model can effectively capture the dynamics without abrupt changes or discontinuities.
without abrupt change or discontinuity.
This smoothness suggests that the dynamics can be identified with a relatively small amount of training data.
\par
\begin{figure*}[tbph]
    \input{figures_greedy_sampling.tex}
    \caption{Gaussian-process based greedy sampling:
    (a) solution uncertainty (\ref{eq:uq-metric}) and
    (b) relative error (\ref{eq:rel-error}) compared to the ground truth at the 14-th iteration;
    (c) relative error (\ref{eq:rel-error}) at the 15-th iteration with an additionally sampled training data point;
    and (d) relative error (\ref{eq:rel-error}) from uniformly sampled initial data as the reference.
    The training data at the current outer-loop iteration is marked with a black box,
    and the initial training data is marked with a red box.}
    \label{fig:greedy-sampling}
\end{figure*}
The uncertainties (\ref{eq:gp-predict}) of all coefficients is
then forward-propagated to HE temperature.
The propagated solution uncertainty (\ref{eq:uq-metric})
is visualized in Figure~\ref{fig:greedy-sampling}~(a).
While the solution uncertainty correlates strongly with the coefficient uncertainty (Figure~\ref{fig:gp-uncertainty}b),
it also reflects the nonlinear dependence of the latent dynamics eigenvalues on the coefficients. 
% Since the eigenvalues of the latent dynamics (\ref{eq:lasdi})
% depend nonlinearly upon the dynamics coefficients,
% the solution uncertainty slightly deviates from
% the coefficient uncertainty shown in Figure~\ref{fig:gp-uncertainty}~(b).
% Nonetheless, the solution uncertainty shown in Figure~\ref{fig:greedy-sampling}~(a)
% exhibits a strong correlation with the coefficient uncertainty.
\par
Figure~\ref{fig:greedy-sampling}~(b) shows the relative error of LaSDI prediction
compared to the ground truth,
\begin{equation}\label{eq:rel-error}
\epsilon[\bT(\bp)]
=
\max_k\frac{\Vert T_k(\bp) - T_{k, pred}(\bp) \Vert_2}{\Vert T_k(\bp) \Vert_2},
\end{equation}
where the maximum value is taken over all timesteps.
We emphasize that, in the absence of the ground truth data,
this relative error is unavailable.
The solution uncertainty (\ref{eq:uq-metric})
exhibits a remarkably strong correlation with the relative error,
though evaluated without the ground truth.
\par
This demonstrates the utility of the solution uncertainty as an error metric for guiding greedy sampling.
Figure~\ref{fig:greedy-sampling}~(c) shows the relative error
after the next 15th outer-loop iteration,
where the new training data point $(p_1, p_2) = (\deg{0}, 1.16\mu m)$
is added based on the solution uncertainty from the 14th outer loop iteration (Figure~\ref{fig:greedy-sampling}a).
Compared to the previous iteration (Figure~\ref{fig:greedy-sampling}b),
the overall prediction accuracy improved dramatically,
achieving a relative error of $\lesssim9\%$ in all test cases.
For comparison,
a reference case was trained using a uniformly sampled dataset of 36 parameter points arranged as a 
$6\times6$ grid over the parameter space $[\deg{0}, \deg{20}]\times [1\mu m, 1.2\mu m]$.
This reference case did not employ greedy sampling, and the inner-loop training was performed for 
$3\times10^4$ iterations---equivalent to the total number of inner-loop iterations in the greedy sampling case.
As shown in Figure~\ref{fig:greedy-sampling}~(d),
the prediction from this uniform sampling achieved a relative error of $\lesssim 8\%$ across all test cases.
Remarkably, the GP-based greedy sampling approach achieved comparable accuracy
with only half the amount of training data, underscoring its efficiency in data-scarce scenarios.
\par
\begin{figure}[tbph]
    \input{figures_metrics.tex}
    \caption{The worst case prediction $(\deg{12}, 1.2\mu m)$ from greedy-sampling training:
    (a) hot spot area ($T>800K$);
    (b) pore area;
    and (c) maximum temperature.}
    \label{fig:metrics}
\end{figure}
Three key metrics are evaluated to assess the prediction accuracy of the trained latent dynamics model.
First, instantaneous hot spot area is calculated with the threshold temperature $800K$,
\todo[inline]{Chris/Keo, can you confirm $800K$ is appropriate threshold temperature?}
\begin{equation}
A_{hotspot}(t_k; \bp) =
\int_{\rD} \mathbf{1}_{T_k(\bx;\bp)>800}(\bx)\;d\bx^2,
\end{equation}
the instantaneous pore area,
\begin{equation}
A_{pore}(t_k; \bp) =
\int_{\rD} \mathbf{1}_{T_k(\bx;\bp)=0}(\bx)\;d\bx^2,
\end{equation}
and the instantaneous maximum temperature
\begin{equation}
T_{k, max}(\bp) = \max_{\bx}T_k(\bx; \bp).
\end{equation}
Figure~\ref{fig:metrics} shows these metrics for the worst case prediction from the greedy sampling case,
corresponding to $(p_1, p_2) = (\deg{12}, 1.2\mu m)$,
which achieved a relative error of approximately $9.3\%$.
The predicted hot spot area and pore area closely match the ground truth,
while the peak of the maximum temperature is slightly underestimated.
For the hot spot area and the pore area,
the prediction matches closely with the ground truth.
This underestimation is likely due to the highly localized and transient nature of the temperature peak,
which may be smoothed during the embedding process in the latent space.
Nevertheless, the model accurately predicts the timing of the peak temperature and the subsequent evolution,
which are critical for upscaling HE material properties.
\par
\begin{figure*}[tbph]
    \input{figures_prediction.tex}
    \caption{Ground truth (left), prediction (middle), and the error (right) of the worst case prediction $(\deg{12}, 1.2\mu m)$ from greedy-sampling training at
    (a) $t=0.2ns$
    (b) $t=0.4ns$
    (c) $t=0.6ns$
    and (d) $t=1.2ns$.
    Errors due to pore mask mis-prediction are marked as white (right).\YC{Can we have snapshots for $t=0.1ns$, $t=0.3ns$,$t=0.5ns$ as well? Just to show more smooth progress of pore collapse process.}}
    \label{fig:prediction}
\end{figure*}
Figure~\ref{fig:prediction}
compares the predicted and ground truth temperature fields for the worst-case prediction at various timesteps.
The latent dynamics model qualitatively captures the evolution of the pore shape and the hot spot after pore collapse.
Aside from pore shape mis-prediction, errors are primarily localized near the shock front
and the boundaries of the hot spots, where physical discontinuities in temperature are present.
These errors are attributed to the spectral bias of the autoencoder,
though these physical discontinuities are much milder than those at the pore boundary.
The maximum point-wise error reaches approximately $147K$
as the pore collapses and hot spot formation,
but decreases down to about $30K$ as the hot spot dissipates.
Despite these localized errors,
the latent dynamics model effectively predicts both the detailed instantaneous evolution
of the temperature and the pore, and the key metrics required for HE material design.

